UCLID5: Multi-Modal Formal Modeling, Verification, and Synthesis

UCLID5 is a tool for the multi-modal formal modeling, verification, and synthesis of systems. It enables one to tackle verification problems for heterogeneous systems such as combinations of hardware and software, or those that have multiple, varied specifications, or systems that require hybrid modes of modeling. A novel aspect of \uclid is an emphasis on the use of syntax-guided and inductive synthesis to automate steps in modeling and verification. This tool paper presents new developments in the \uclid tool including new language features, integration with new techniques for syntax-guided synthesis and satisfiability solving, support for hyperproperties and combinations of axiomatic and operational modeling, demonstrations on new problem classes, and a robust implementation.

==> figures/control_minimal.tex <==
module main {
  var x0, x1: float;
  group states : float = {x0, x1};
  <..LTI system spec vars decls..>
  oracle function [isstable] isStable
    (s00:float, s01:float, s10:float, s11:float) : boolean;
  synthesis function k0 (): float;
  synthesis function k1 (): float;

  // LTI system spec values
  axiom A:(a00==0.901224922471 && a01==0.000000013429 && a10==0.000000007451 && a11==0.0);
  axiom B: (b0==128.0 && b1==0.0);
  axiom ax1: ABK00 == a00 - b0*k0());
  <...>
  axiom ax4: ABK11 == a11 - b1*k1());

  init { // bound initial states
    assume (finite_forall (s: float) in states :: s<0.1 && s>-0.1);
  }
  next { // step the system
    x0' = ABK00*x0 + ABK01*x1;
    x1' = ABK10*x0 + ABK11*x1;
  }
  // the safety condition
  invariant stability: isStable(ABK00, ABK01, ABK10, ABK11);
  invariant safety: finite_forall (s: float) in states :: s < 1.0&&s > -1.0;

  control {
    unroll(10); // fix safety bound
    check;
  }
}

==> figures/cpu.tex <==
module common {
// common types
}

module cpu {
  // import all types from module common
  type * = common.*;

  type regindex_t;
  type regs_t = [regindex_t]word_t;

  input imem         : mem_t;  // program memory.
  var dmem           : mem_t;  // data memory.
  var regs           : regs_t; // registers.
  var pc             : addr_t; // program counter.
  var inst, result   : word_t; // inst reg, result
  var mode           : mode_t; // normal/isolated mode?

  // rng of isolated memory.
  const isolated_rng_lo, isolated_rng_hi : addr_t;
  // uninterpreted func. (predicate) for the above.
  function in_rng  (a : addr_t, b1 : addr_t, b2 : addr_t) : boolean;
  // uninterpreted functions for decoding insns.
  function inst2op 
    (i : word_t) : op_t;
  function inst2reg0 
    (i : word_t) : regindex_t;
  ...

  // macro: is an addr in isolated memory?
  define in_isolated_memory (a : addr_t) : boolean 
          = in_rng(a, isolated_rng_lo, isolated_rng_hi);

  // assumptions on imode entry and exit addresses
  axiom (forall (a : addr_t) :: 
          (a == common.imode_enter_addr) 
              ==> in_isolated_memory(a));
  axiom (forall (a : addr_t) :: 
          (a == common.nmode_exit_addr) 
              ==> !in_isolated_memory(a));

  procedure exec_inst(instr : word_t, pc : addr_t)
    returns (pc_next : addr_t)
    modifies regs, result, dmem, mode;
  {
   // sequential code that executes the instruction
  }
  init {
    // initialise registers and mode
  }

  next {
    inst' = imem[pc];
    call (pc') = exec_inst(inst', pc);
  }
}

module main {
  // Import types.
  type * = common.*;
  type regindex_t = cpu.regindex_t;

  // Instruction memory for the CPUs.
  var imem1, imem2 : mem_t;

  // Create two instances of the CPU module.
  instance cpu1 : cpu(imem : (imem1));
  instance cpu2 : cpu(imem : (imem2));

  init {
    // Assume same isolated rngs.
    assume (cpu1.isolated_rng_lo == cpu2.isolated_rng_lo);
    assume (cpu1.isolated_rng_hi == cpu2.isolated_rng_hi);
    // Supervisor memory starts off identical.
    assume (forall (a : addr_t) :: (cpu.in_rng(a, cpu1.isolated_rng_lo, cpu2.isolated_rng_hi)) ==> (cpu1.dmem[a] == cpu2.dmem[a]));
    assume (forall (a : addr_t) :: (cpu.in_rng(a, cpu1.isolated_rng_lo, cpu1.isolated_rng_hi)) ==> (imem1[a] == imem2[a]));
  }

  next {
    next (cpu1);  next (cpu2);
    // imodes are taken in sync
    assume (cpu.inst2op(cpu1.inst) == op_imode_enter || cpu.inst2op(cpu2.inst) == op_imode_enter) ==> (cpu1.inst == cpu2.inst);
  }

  // PROPERTY: isolated mode memory is identical.
  property eq_dmem : (forall (a : addr_t) :: (cpu.in_rng(a, cpu1.isolated_rng_lo, cpu2.isolated_rng_hi)) ==> (cpu1.dmem[a] == cpu2.dmem[a]));
  // The two CPUs change mode in sync.
  invariant eq_mode : (cpu1.mode == cpu2.mode);
  ...
  control {
    v = induction;
    check;
  }
}


==> figures/hyper.tex <==
module main
{
    var x, y : integer;
    init { y = x + 1;}
    next { y' = y + 1;}
    hyperaxiom[2] x_eq: x.1 == x.2;
    hyperinvariant[2] det_xy: y.1 == y.2;
}

==> figures/prime.tex <==
module main {
  var a : [integer]integer;
  oracle function [isprime] isPrime(x: integer) : boolean;
  var count, i : integer
  init { count,i=0; }
  next {
    if(isprime(a[i]) && i < 20)
    {  count' = count++; }
    i'=i++
  }
  invariant all_prime: count==i;
  control {
    unroll(20);
    check;
  }
}

==> related.tex <==
% point to original uclid5 paper for broader comparison


% \todo[inline]{Federico, Kevin}
% \todo[inline]{draw contrast: e.g., modelling concurrent systems with boogie needs you to explicitly model synchronisation}
% % https://link.springer.com/chapter/10.1007/978-3-030-81688-9_22

% % Higher level of abstraction then writing formulas, like you do in SMT directly. There is value in providing axiomatic modelling at a higher level of abstraction than SMT. 

% % Blending axiomatic and operational modeling is rare (according to Yatin) (counterexample to that is Ivy).

There are a multitude of verification and synthesis tools related to \uclid{}. In this brief review, we highlight prominent examples and contrast them with \uclid{} along the key language features described in Section~\ref{sec:features}. 

\uclid{} allows users to combine sequential and concurrent modeling (see Section~\ref{sec:seq-concur}). Most existing tools primarily support either sequential, e.g. \cite{dafny,boogie,rosette}, or concurrent computation modeling, e.g. \cite{abc,nuxmv,ivy,sally,pono}. Users of these systems can often overcome the tool's modeling focus by manually including support for different computation paradigms. For example, Dafny can be used to model concurrent systems \cite{dafny-concurrent}. Unfortunately, this is not always straightforward, and limited support for different paradigms can manifest as limitations in downstream applications. For example, the Serval~\cite{serval} framework, based on Rosette, cannot reason about concurrent code.

\uclid{} supports different kinds of specifications and verification procedures (see Section~\ref{sec:verification_modes}). Most existing tools do no support multi-modal verification at all, e.g. \cite{dafny,abc,nuxmv}. Tools that do offer multi-modal verification do not offer the same range of options as \uclid{}. For example, \cite{pono} does not support linear temporal logic, and \cite{ivy,murphi} does not support hyper property verification.

% \uclid{} supports satisfiability modulo oracles (see Section~\ref{sec:smto}).

Finally, \uclid{} supports a generic integration with program synthesis (see Section~\ref{sec:synthesis}). This makes \uclid{} related to a number of synthesis engines. 
The SKETCH system~\cite{solar2009} synthesizes expressions to fill holes in programs, and has subsequently been applied to program repair~\cite{DBLP:conf/icse/HuaZWK18}. \uclid{} aims to be more flexible than this work, allowing users to declare unknown functions even in the verification annotations, as well as supporting multiple verification algorithms and types of properties.
Rosette~\cite{rosette} provides support for synthesis and verification, but, unlike \uclid{}, the synthesis is limited
to bounded specifications of sequential programs and there is no support for external synthesis engines.
Synthesis algorithms have been used to assist in verification tasks, such as safety and termination of loops~\cite{DBLP:conf/lpar/DavidKL15}, and generating invariants~\cite{DBLP:conf/tacas/FedyukovichB18,DBLP:conf/vmcai/ZhangYFGM20}, but none
of this work to-date integrates program synthesis fully into an existing verification tool. 
Before the new synthesis integration, \uclid{} supported synthesis of inductive invariants. The key insight of this work is to generalize the synthesis support, and to unify all synthesis tasks by re-using the verification back-end.

% Not sure what to say about combining axiomatic and operational. Most systems let you use axioms or assumptions. For example, verilog lets you assume properties so tools like Pono that accept verilog give you this same functionality. Other tools like nuxmv might be slightly less pleasant for this purpose, but it really does seem like assumptions are a fundamental thing that most tools support. 

% Instead of writing "axiom <expr>;" like we do in uclid, they write "assume property (<expr>);" 

==> sections/synthesis.tex <==
% USIR? Change the synth-lib name
% Move background stuff to arch?

\subsection{Integration with Synthesis}
% \todo[inline]{Elizabeth, Federico}
\label{sec:synthesis}
UCLID5 integrates program synthesis fully across all verification modes described in section~\ref{sec:verification_modes}. Specifically, users can declare and use \emph{synthesis functions} anywhere in their models, and UCLID5 will automatically synthesize function bodies for these functions such that the user-selected verification task will pass by deploying a syntax-guided synthesis solver. 
%
Specifically, given a \uclid model in which the user has declared a function to synthesize, $f$, we build a synthesis query $\exists f \; \forall \vec{x}\; \bigwedge_{i=0}^{i=n} P_i(f, \vec{x})$
where each $P_i$ encodes a verification condition that may refer to the function to synthesize, $f$. We then use a SyGuS solver to check its validity.
%
This scheme lets us enable synthesis for any verification procedure in \uclid, by simply letting users declare and use functions to synthesize and relying on existing \sygusif solvers to carry out the automated reasoning.

% In this section, we give an illustrative example of synthesis in \uclid, we provide the necessary background on program synthesis, and then we formulate the existing verification techniques inside of \uclid for synthesis.

% \subsubsection{Synthesis Example}
\paragraph{Synthesis Example:} Consider the \uclid model in Fig.~\ref{ex:fib}, which represents a Fibonacci sequence. 
The (hypothetical) user wants to prove by induction that the invariant \codelike{a\_le\_b} at line 13 always holds. Unfortunately, the proof fails because the invariant is not inductive. Without synthesis, the user would need to manually strengthen the invariant until it became inductive. However, the user can ask \uclid to automatically do this for them. Fig.~\ref{ex:fib} demonstrates this on lines 16, 17 and 18. Specifically, the user specifies a function to synthesize called \codelike{h} at lines 16 and 17, and then uses \codelike{h} at line 18 to strengthen the existing set of invariants. Given this input, \uclid, using e.g. \textsc{cvc5}~\cite{cvc4} as a synthesis engine, will automatically generate the function \codelike{h(x, y) = x >= 0}, which completes the inductive proof. 

In this example, the function to synthesize represents an inductive invariant. However, functions to synthesize are treated exactly like any interpreted function in \uclid: the user could have called \codelike{h} anywhere in the code. Furthermore, this example uses induction and a global invariant, however, the user could also have used a linear temporal logic (LTL) specification and bounded model checking (BMC). In this sense, our integration is fully flexible and generic.

\begin{figure}[t]
  \lstinputlisting[language=uclid,style=uclidstyle]{figures/example.tex}
  \caption{\uclid Fibonacci model. Part 3 shows the new synthesis syntax, and how to find an auxiliary invariant.}
  \label{ex:fib}
\end{figure}
  
% \subsubsection{Synthesis Encoding in \uclid}\label{sec:encoding}
% The program synthesis problem corresponds to the second-order query $\exists f\; \forall \vec{x} \sigma(f, \vec{x}) \label{eq:sygus},$ where $f$ is the function to synthesize, $\vec{x}$ is the set of all possible inputs, and $\sigma$ is the specification to be satisfied. 

% \subsubsection{Verification in \uclid Formulated For Synthesis}
% At at high level, \uclid takes in a model, generates a set of verification conditions, asks a satisfiability modulo theory (SMT) solver~\cite{barrett-smtbookch09} to check the verification conditions, and then returns the results to the user. This process is the same regardless of the proof procedure used. The important point, is that \uclid encodes the violation of each independent verification condition as a separate \smtlib query.

% Let $P_i(\vec{x})$ encode the $i^{th}$ verification condition, and take the $i^{th}$ \smtlib query to be checking the validity of $\exists \vec{x} \; \neg P_i(\vec{x})$, where $P_i$ contains no free variables. 
% We say that there is a counterexample to the $i^{th}$ verification query if the query $\exists \vec{x} \; \neg P_i(\vec{x})$ is valid. Verification of a model with $n$ verification conditions succeeds \emph{iff} there are no counter-examples:
% $$\forall \vec{x}\; \bigwedge_{i=0}^{i=n} P_i(\vec{x}).$$

% Given a \uclid model in which the user has declared a function to synthesize, $f$, we wish to construct a synthesis query that is satisfied \emph{iff}
% there is an $f$ for which all the verification conditions pass for all possible inputs. We build this synthesis query by taking the conjunction of the negation of all the verification queries. Specifically, we generate the query
% $\exists f \; \forall \vec{x}\; \bigwedge_{i=0}^{i=n} P_i(f, \vec{x})$
% where each $P_i$ encodes a verification condition that may refer to the function to synthesize, $f$, and then we use a SyGuS solver to check its validity.

% This scheme lets us enable synthesis for any verification procedure in \uclid, by simply letting users declare and use functions to synthesize and relying on existing \sygusif solvers to carry out the automated reasoning.

\subsubsection{Synthesis Modulo Oracles} UCLID5 supports synthesis modulo oracles in the same way as it support satisfiability modulo oracles, i.e., a user can specify oracle functions (functions whose implementation is provided as an external oracle) and use these throughout a UCLID5 model. When the synthesis command is used, UCLID5 will produce a file in the \sygusif format that includes oracle functions. We note that oracle functions (and functions in general) can only be first-order within the UCLID5 modeling language, i.e., functions cannot receive functions as arguments. 


As a more elaborate example of the UCLID5 synthesis integration, combined with oracles, consider the task of synthesising a controller for a Linear Time Invariant similar to Abate et al.~\cite{control-cegis}. We use a state-space representation, which is discretized in time:
%
$
\label{eq:ode1}
\dot{x}_{t+1} = \mat{A}\vec{x}_t+ \mat{B} \vec{u}_t, 
$
%
where 
$\vec{x} \in \mathbb{R}^n$,  
$\vec{u} \in \mathbb{R}^p$ is the input to the system, calculated as $\mat{K}\vec{x}$ where $\mat{K}$ is the controller to be synthesized, 
$\mat{A} \in \mathbb{R}^{n \times n}$ is the system matrix, 
$\mat{B} \in \mathbb{R}^{n \times p}$ is the input matrix,
and subscript $t$ indicates the discrete time step. 

We aim to find a stabilizing controller, such that absolute values of the (potentially complex) eigenvalues of the closed-loop matrix 
$\mat{A} - \mat{B}\mat{K}$
are less than one. We further require that the controller guarantees the states remain within a safe region of the state space up to a given number of time steps, using the bounded model checking verification command in UCLID5, as shown in Figure~\ref{ex:control}.

\begin{figure}
  \lstinputlisting[language=uclid,style=uclidstyle]{figures/control_minimal.tex}
  \caption{\uclid control synthesis example. The next block assigns to the state variables according to Equation~\ref{eq:ode1}. Note this model uses finite quantifiers, as described in Section~\ref{sec:axiom}.
  \label{ex:control}}
\end{figure}



